Smoothing Policy Iteration for Zero-sum Markov Games

Zero-sum Markov Games (MGs) has been an efficient framework for multi-agent systems and robust control, wherein a minimax problem is constructed to solve the equilibrium policies. At present, this formulation is well studied under tabular settings wherein the maximum operator is primarily and exactly solved to calculate the worst-case value function. However, it is non-trivial to extend such methods to handle complex tasks, as finding the maximum over large-scale action spaces is usually cumbersome. In this paper, we propose the smoothing policy iteration (SPI) algorithm to solve the zero-sum MGs approximately, where the maximum operator is replaced by the weighted LogSumExp (WLSE) function to obtain the nearly optimal equilibrium policies. Specially, the adversarial policy is served as the weight function to enable an efficient sampling over action spaces.We also prove the convergence of SPI and analyze its approximation error in $\infty -$norm based on the contraction mapping theorem. Besides, we propose a model-based algorithm called Smooth adversarial Actor-critic (SaAC) by extending SPI with the function approximations. The target value related to WLSE function is evaluated by the sampled trajectories and then mean square error is constructed to optimize the value function, and the gradient-ascent-descent methods are adopted to optimize the protagonist and adversarial policies jointly. In addition, we incorporate the reparameterization technique in model-based gradient back-propagation to prevent the gradient vanishing due to sampling from the stochastic policies. We verify our algorithm in both tabular and function approximation settings. Results show that SPI can approximate the worst-case value function with a high accuracy and SaAC can stabilize the training process and improve the adversarial robustness in a large margin.

==> latex/2Related_works.tex <==
\section{Related works}
In this section, we introduce the framework of integrated decision and control (IDC). As shown in Fig., the framework consists of two layers: static path planning and dynamic optimal tracking.

Different from existing schemes, the upper layer aims to generate multiple candidate paths only considering static information such as road structure, speed limit, traffic signs and lights. Note that these paths will not include time information. Each candidate path is attached with an expected velocity determined by rules from human experience. Similar to existing trajectory planning methods, there is no optimality guarantee with the path generation. However, the time complexity of the path selection in our method remains unchanged with the growth of the candidate path set. Therefore, we can increase the number of reference paths according to our demand until the required performance is met. For example, at intersection, the candidate path can be as many as the number of the exit lanes; on highway, the candidate path can include the centerline of the current and adjacent lanes, etc.

The lower layer further considers the candidate paths and the dynamic information such as surrounding vehicles, pedestrians and bicycles. For each candidate path, a constrained optimal control problem (OCP) is formulated and optimized to choose the optimal path and find the control command. The objective function is to minimize the tracking error within a finite horizon and the constraints characterize safety requirements. In each time step, the optimal path is chosen as the one with the lowest optimal cost function and thereafter tracked. The core of our method is to substitute all the expensive online optimizations with feed-forward of two neural networks (NNs) trained offline by reinforcement learning (RL). Specifically, we first formulate a complete RL problem considering all the candidate paths. And then we develop a model-based RL algorithm to solve this problem to obtain a policy NN called actor that is capable of tracking different shape of paths while maintaining the ability to avoid collisions. Meanwhile, a value NN called critic is learned to approximate the optimal cost of tracking different paths, for the purpose of online path selection.
% \begin{figure*}[!htb]
% \centering{\includegraphics[width=0.7\textwidth]{figure/framework.pdf}}
% \caption{Illustration of the integrated decision and control framework.}
% \label{fig.overall_framework}
% \end{figure*}

The advantages of the IDC framework are summarized in three points. 
First, it has high online computing efficiency. The upper layer can be quite efficient because it involves only static information. It even allows to embed key path parameters into the electronic map. On the other hand, the lower layer utilizes two trained networks to compute optimal path and control command, which is also time-saving due to the fast propagation of NNs.
Second, it can be easily transferred among different driving scenarios without a lot of human design. As the upper layer only uses the static information, the multiple paths can be easily generated by the road topology of various scenes such as intersections, roundabouts and ramps. Besides, the lower-layer always formulates a similar tracking problem with safety constraints no matter what the task is, which all can be solved by the developed model-based solver, saving time to design separate reward functions for different tasks.
Third, the IDC framework has great interpretability. Interpretability is defined as the degree to which a human can understand the cause of a decision \cite{miller2019explanation} or the degree to which a human can consistently predict the model’s result \cite{kim2016examples}. The IDC is interpretable in the way that the learned value and policy functions are approximation to the optimal value and the optimal action of the constrained OCPs. The path selection result is expected to be the candidate path that has the least optimal objective value among all the candidates. And the path tracking result is expected to be the optimal action of the OCP corresponding to the optimal path. These results can be understood from the construction of the OCPs and exactly predicted using model predictive control (MPC) methods.

==> latex/6realtests.tex <==
\section{Real vehicle experiments}
\label{sec.real_vehciel_experiments}
This section deploys the proposed method on real vehicle experiments at a signalized intersection to verify its effectiveness and robustness against abnormal behaviors.

\subsection{Experimental description}
\begin{figure}[!htbp]
\captionsetup[subfigure]{justification=centering}
\subfloat[Experimental vehicle\label{fig.experimental_vehicle}]{\includegraphics[width=0.421\linewidth]{figure/exp_vehicle.jpg}}
\subfloat[Experimental site\label{fig.experimental_site}]{\includegraphics[width=0.5\linewidth]{figure/exp_site.png}}
\caption{Equipment and site of real vehicle experiments}
\label{fig.equip_&_site_real_veh_exp}
\end{figure}

Fig.~\ref{fig.equip_&_site_real_veh_exp} shows the experimental equipment and site conditions. The utilized vehicle is the Volvo XC60, a sport utility vehicle equipped with one 64-channel lidar, two 16-channel lidars, seven cameras, and twelve radars. 
Its driving system can switch between automatic driving and manual driving, and a safety supervisor will take over the vehicle immediately in case of an emergency.
The experiment site is a signalized irregular intersection located at (39.09172$\degree$N, 117.43920$\degree$E) in Dongli distinct, Tianjin, China. The intersection is 60m long in the east-west direction with four lanes at the entrance and three lanes at the exit, while it is 65m long in the south-north direction, featured with two-way six-lane motor traffic. Besides, there is a non-motor lane in each direction. For all experiments, the experimental vehicle departs from the south and attempts to pass this intersection under the guidance of traffic lights. Therefore, according to the principle of static path planning and the road topology, the numbers of alternative routes for left-turn, straight-going, and right-turn tasks are set as 3, 2, and 3, respectively. In addition, speed limits inside and outside the intersection are set as 4m/s and 5m/s, respectively.
There is actual traffic flow in this intersection, where human drivers steer the other six vehicles. Additionally, nine pedestrians and three bicyclists attempt to pass this intersection following the signal lights. 

\begin{figure}[!htbp]
\includegraphics[width=0.99\linewidth]{figure/pipeline_real_veh_exp.pdf}
\caption{Pipeline of real vehicle experiments}
\label{fig.real_veh_pipeline}
\end{figure}

The experimental pipeline is demonstrated in Fig.~\ref{fig.real_veh_pipeline}. An onboard industrial personal computer (IPC) takes charge of all calculations, equipped with one 12-core Intel$^\circledR$ Xeon Gold 6146 CPU, two Nvidia$^\circledR$ GeForce GTX 1070 GPUs, and 2 Nvidia$^\circledR$ Tesla T4 Tensor Core GPUs. 
The localization module includes differential GPS (DGPS) and high definition map (HD Map), which can provide location and navigation information for the ego vehicle. 
The perception module captures the information of surrounding participants and traffic lights, which is then fused and inputted into the IDC module. 
The value network calculates the optimal value indicating the current optimal path, and then the policy network outputs optimal control commands and sends them to the actuator by CAN Bus. 
As for the practical scheme, we firstly construct a simulation based on the HD Map of the experimental intersection and simulated traffic flow, where both the value network and the policy network are trained. After that, we evaluate the policy performance under a high-fidelity dynamical model to verify safety. Finally, we compile and deploy the two networks on the IPC to carry out all experiments.

\subsection{Experimental results}
Four experiments are conducted to verify the effectiveness and robustness of the proposed method under abnormal scenarios, where all traffic participants are dispatched to ensure the procedures are the same as design.

Fig.~\ref{fig.real_exp1_traj} shows an autonomous driving process of a left turn, where a pedestrian suddenly turns back to the zebra crossing. The ego vehicle firstly tracks the second static path and stops at the zebra crossing waiting for pedestrians to pass, as shown in Fig.~\ref{fig.real_exp1_237}. After pedestrians pass the zebra crossing, the ego vehicle starts to accelerate and aims to leave the intersection, as shown in Fig.~\ref{fig.real_exp1_281}. However, from Fig.~\ref{fig.real_exp1_296}, a pedestrian suddenly turns back to the zebra crossing and immediately catches the attention of the ego vehicle. Reasonably, the ego vehicle brakes persistently to avoid the collision, as shown in Fig.~\ref{fig.real_exp1_307}. In addition, the emergency brake is demonstrated in the gray shaded areas of Fig.~\ref{fig.real_exp1_v_x}, where the longitudinal velocity quickly decreases to zero at 30.7s.

\begin{figure}[!htbp]
\centering
\captionsetup[subfigure]{justification=centering}
\subfloat[t=23.7s]{\label{fig.real_exp1_237}\includegraphics[width=0.4\linewidth]{figure/real_exp1/237.pdf}} \,
\subfloat[t=28.1s]{\label{fig.real_exp1_281}\includegraphics[width=0.4\linewidth]{figure/real_exp1/281.pdf}}
\\
\subfloat[t=29.6s]{\label{fig.real_exp1_296}\includegraphics[width=0.4\linewidth]{figure/real_exp1/296.pdf}} \,
\subfloat[t=30.7s]{\label{fig.real_exp1_307}\includegraphics[width=0.4\linewidth]{figure/real_exp1/307.pdf}} \,
\caption{The 1st experiment: trajectory visualization. The pink box represents the ego vehicle controlled by the trained policy. The highlighted curve is the current chosen static path. The bold pink curve is the historical trajectory of the ego vehicle, where darker pink means longer staying time. The black boxes indicate surrounding vehicles, while the purple boxes denote pedestrians and bicyclists. Objects catching the attention of the ego vehicle are filled with blue, whereas darker blue means more attention. Critical objects of this scenario are further emphasized by green arrows.}
\label{fig.real_exp1_traj}
\end{figure}

\begin{figure}[!htbp]
\centering
\captionsetup[figure]{justification=centering}
\includegraphics[width=0.96\linewidth]{figure/real_exp1/demo-v_x.pdf}
\caption{The 1st experiment: longitudinal velocity.}
\label{fig.real_exp1_v_x}
\end{figure}

Fig.~\ref{fig.real_exp2_traj} shows a scenario where a pedestrian in blind spots unexpectedly intrudes into the driving lane. The ego vehicle firstly travels in the right-turn lane, having no pedestrian in view, as shown in Fig.~\ref{fig.real_exp2_020}. Abruptly, a pedestrian appears in front of the preceding vehicle and is going to run across the road, as shown in Fig.~\ref{fig.real_exp2_048}. Observing that, the ego vehicle decreases right away, and the violent braking process is shown in the shaded area of Fig.~\ref{fig.real_exp2_acc}. Note that we display the expected acceleration from the policy network and the actual acceleration of the ego vehicle, between which there is an acceptable operating lag. The ego vehicle stops at 6.5s in Fig.~\ref{fig.real_exp2_065} and re-accelerates to pass the intersection, as shown in Fig.~\ref{fig.real_exp2_083}. We also visualize the sensor information in Fig.~\ref{fig.real_exp2_snapshots}. The ego vehicle drives straight at 2.0s while the pedestrian is blocked by the preceding vehicle. When the pedestrian bursts into the view at 4.8s, the ego vehicle brakes immediately and successfully avoid the collision at 6.5s. We claim that sharing information is the most effective solution to such situations, but the results show that our proposed method can handle them when the vehicle is at low speed.

\begin{figure}[!htbp]
\centering
\captionsetup[subfigure]{justification=centering}
\subfloat[t=2.0s]{\label{fig.real_exp2_020}\includegraphics[width=0.4\linewidth]{figure/real_exp2/020.pdf}} \,
\subfloat[t=4.8s]{\label{fig.real_exp2_048}\includegraphics[width=0.4\linewidth]{figure/real_exp2/048.pdf}}
\\
\subfloat[t=6.5s]{\label{fig.real_exp2_065}\includegraphics[width=0.4\linewidth]{figure/real_exp2/065.pdf}} \,
\subfloat[t=8.3s]{\label{fig.real_exp2_083}\includegraphics[width=0.4\linewidth]{figure/real_exp2/083.pdf}}
\caption{The 2nd experiment: trajectory visualization.}
\label{fig.real_exp2_traj}
\end{figure}

\begin{figure}[!htbp]
\centering
\captionsetup[figure]{justification=centering}
\includegraphics[width=0.96\linewidth]{figure/real_exp2/demo-acc.pdf}
\caption{The 2nd experiment: acceleration.}
\label{fig.real_exp2_acc}
\end{figure}

\begin{figure}[!htbp]
\centering
\captionsetup[subfigure]{justification=centering}
\subfloat[t=2.0s]{\label{fig.real_exp2_go_straight}\includegraphics[width=0.32\linewidth]{figure/real_exp2/go_straight.pdf}}\,
\subfloat[t=4.8s]{\label{fig.real_exp2_ped_show}\includegraphics[width=0.32\linewidth]{figure/real_exp2/pedestrain_show.pdf}}\,
\subfloat[t=6.5s]{\label{fig.real_exp2_emerg_brake}\includegraphics[width=0.32\linewidth]{figure/real_exp2/emergency_brake.pdf}}
\caption{The 2nd experiment: snapshots.}
\label{fig.real_exp2_snapshots}
\end{figure}

% Fig~\ref{fig.real_exp3_traj} displays another right-turn scenario where a vehicle illegally and repeatedly changes lanes. In the beginning, the ego vehicle tracks the third static path to reach the zebra crossing and waits for all pedestrians and bicyclists to pass, as shown in Fig.~\ref{fig.real_exp3_152}. The ego vehicle does not start to accelerate until the road ahead is clear, as shown in Fig.~\ref{fig.real_exp3_191}. However, a car running in the north-most lane makes two illegal lane changes abruptly and impedes the movement of the ego vehicle, as shown in Fig.~\ref{fig.real_exp3_230} and Fig.~\ref{fig.real_exp2_048}. Conditioned on that, Fig.~\ref{fig.real_exp3_contr_command} indicates that the ego vehicle decelerates and turns right at around 20s-25s to avoid the obstacle vehicle and finally smoothly drives along the third lane.

% \begin{figure}[!htbp]
% \centering
% \captionsetup[subfigure]{justification=centering}
% \subfloat[t=15.2s]{\label{fig.real_exp3_152}\includegraphics[width=0.4\linewidth]{figure/real_exp3/152.pdf}} \,
% \subfloat[t=19.1s]{\label{fig.real_exp3_191}\includegraphics[width=0.4\linewidth]{figure/real_exp3/191.pdf}}
% \\
% \subfloat[t=23.0s]{\label{fig.real_exp3_230}\includegraphics[width=0.4\linewidth]{figure/real_exp3/230.pdf}} \,
% \subfloat[t=24.8s]{\label{fig.real_exp3_248}\includegraphics[width=0.4\linewidth]{figure/real_exp3/248.pdf}}
% \caption{The 3rd experiment: trajectory visualization.}
% \label{fig.real_exp3_traj}
% \end{figure}

% \begin{figure}[!htbp]
% \centering
% \captionsetup[subfigure]{justification=centering}
% \subfloat[Acceleration]{\label{fig.real_exp3_acc}\includegraphics[width=0.96\linewidth]{figure/real_exp3/demo-acc.pdf}}
% \\
% \subfloat[Steering wheel angle]{\label{fig.real_exp3_steer}\includegraphics[width=0.96\linewidth]{figure/real_exp3/demo-steer.pdf}}
% \caption{The 3rd experiment: control commands.}
% \label{fig.real_exp3_contr_command}
% \end{figure}

Fig.~\ref{fig.real_exp3_traj} demonstrates a left-turn scenario where the preceding vehicle emergency brakes. In Fig.~\ref{fig.real_exp3_000}, the ego vehicle initially selects the second static path as its tracking reference. Then, to bypass the prior vehicle, the ego vehicle changes its static reference path to the third one, as shown in Fig.~\ref{fig.real_exp3_169}. Unexpectedly, a pedestrian is going to runs across the road and forces the preceding vehicle to stop. Meanwhile, because the opposite car is approaching continually, there is less room for the ego vehicle to pass through, see Fig.~\ref{fig.real_exp3_184}. Fig.~\ref{fig.real_exp3_state&action} indicates that the ego vehicle brakes and turns left immediately to keep clear of the opposite vehicle under this emergency. Finally, after the preceding vehicle restarts, the ego vehicle accelerates and drives along the straight road almost side by side with the other two, with the attention focusing on either of them, as shown in Fig.~\ref{fig.real_exp3_209}, Fig.~\ref{fig.real_exp3_248}, and Fig.~\ref{fig.real_exp3_293}.

\begin{figure}[!htbp]
\centering
\captionsetup[subfigure]{justification=centering}
\subfloat[t=0.0s]{\label{fig.real_exp3_000}\includegraphics[width=0.32\linewidth]{figure/real_exp3/000.pdf}} \, 
\subfloat[t=16.9s]{\label{fig.real_exp3_169}\includegraphics[width=0.32\linewidth]{figure/real_exp3/169.pdf}} \,
\subfloat[t=18.4s]{\label{fig.real_exp3_184}\includegraphics[width=0.32\linewidth]{figure/real_exp3/184.pdf}}
\\
\subfloat[t=20.9s]{\label{fig.real_exp3_209}\includegraphics[width=0.32\linewidth]{figure/real_exp3/209.pdf}} \,
\subfloat[t=24.8s]{\label{fig.real_exp3_248}\includegraphics[width=0.32\linewidth]{figure/real_exp3/248.pdf}} \,
\subfloat[t=29.3s]{\label{fig.real_exp3_293}\includegraphics[width=0.32\linewidth]{figure/real_exp3/293.pdf}}
\caption{The 3rd experiment: trajectory visualization.}
\label{fig.real_exp3_traj}
\end{figure}

\begin{figure}[!htbp]
\centering
\captionsetup[subfigure]{justification=centering}
\subfloat[Longitudinal velocity]{\label{fig.real_exp3_v_x}\includegraphics[width=0.96\linewidth]{figure/real_exp3/demo-v_x.pdf}}
\\
\subfloat[Acceleration]{\label{fig.real_exp3_acc}\includegraphics[width=0.96\linewidth]{figure/real_exp3/demo-acc.pdf}}
\\
\subfloat[Steering wheel angle]{\label{fig.real_exp3_steer}\includegraphics[width=0.96\linewidth]{figure/real_exp3/demo-steer.pdf}}
\caption{The 3rd experiment: state and control commands.}
\label{fig.real_exp3_state&action}
\end{figure}

A straight-going task is shown in Fig.~\ref{fig.real_exp4_traj}, where the preceding vehicle intentionally brakes and swerves to block the ego. The ego vehicle aims to go straight through the intersection at the start. However, the prior brakes and swerves suddenly, and the ego vehicle turns right correspondingly for collision avoidance, see Fig.~\ref{fig.real_exp4_095}1 and Fig.~\ref{fig.real_exp4_120}. Once the preceding vehicle gets out of the way, the ego vehicle precisely tracks the static path, as shown in Fig.~\ref{fig.real_exp4_150}. Latter, the prior turns right again, and the ego vehicle makes another reasonable avoidance, as shown in Fig.~\ref{fig.real_exp4_170}. Finally, the steering wheel angle of the ego vehicle is displayed in Fig.~\ref{fig.real_exp4_steer}, showing two urgent right turns at around 10s and 17s.

\begin{figure}[!htbp]
\centering
\captionsetup[subfigure]{justification=centering}
\subfloat[t=9.5s]{\label{fig.real_exp4_095}\includegraphics[width=0.4\linewidth]{figure/real_exp4/095.pdf}} \,
\subfloat[t=12.0s]{\label{fig.real_exp4_120}\includegraphics[width=0.4\linewidth]{figure/real_exp4/120.pdf}}
\\
\subfloat[t=15.0s]{\label{fig.real_exp4_150}\includegraphics[width=0.4\linewidth]{figure/real_exp4/150.pdf}} \,
\subfloat[t=17.0s]{\label{fig.real_exp4_170}\includegraphics[width=0.4\linewidth]{figure/real_exp4/170.pdf}}
\caption{The 4th experiment: trajectory visualization.}
\label{fig.real_exp4_traj}
\end{figure}

\begin{figure}[!htbp]
\centering
\captionsetup[figure]{justification=centering}
\includegraphics[width=0.96\linewidth]{figure/real_exp4/demo-steer.pdf}
\caption{The 4th experiment: steering wheel angle.}
\label{fig.real_exp4_steer}
\end{figure}

In summary, the proposed method realizes relatively safe and smooth decision-making and control under abnormal scenarios, showing fairly well effectiveness and robustness. Moreover, Fig.~\ref{fig.real_exp_decision_time} indicates that the decision time of all experiments is shorter than 6.5ms, meeting the real-time requirements of high-level autonomous driving.

\begin{figure}[!htbp]
\centering
\captionsetup[figure]{justification=centering}
\includegraphics[width=0.85\linewidth]{figure/decision_time_boxplot.pdf}
\caption{Decision time for 4 real vehicle experiments.}
\label{fig.real_exp_decision_time}
\end{figure}
